ScriptSmith: A Unified LLM Framework for Enhancing IT Operations via Automated Bash Script Generation, Assessment, and Refinement

In the rapidly evolving landscape of site reliability engineering (SRE), the demand for efficient and effective solutions to manage and resolve issues in site and cloud applications is paramount. This paper presents an innovative approach to action automation using large language models (LLMs) for script generation, assessment, and refinement. By leveraging the capabilities of LLMs, we aim to significantly reduce the human effort involved in writing and debugging scripts, thereby enhancing the productivity of SRE teams. Our experiments focus on Bash scripts, a commonly used tool in SRE, and involve the CodeSift dataset of 100 tasks and the InterCode dataset of 153 tasks. The results show that LLMs can automatically assess and refine scripts efficiently, reducing the need for script validation in an execution environment. Results demonstrate that the framework shows an overall improvement of 7-10% in script generation.

==> CameraReady/LaTeX/body/ack.tex <==
\section{Acknowledgements}
We thank XXX and XXX of the Instana product team for participating in the user study and providing useful feedback and comments.

==> CameraReady/LaTeX/body/future.tex <==
\section{Future work}



==> CameraReady/LaTeX/body/notes.tex <==
coffeepot paper - see how human evaluations are done

==> CameraReady/LaTeX/body/relatedArt_long.tex <==
\section{Related Work}
\textbf{Benchmarking:} 
Traditional coding benchmarks like NL2Bash~\cite{nl2bash2018}, HumanEval~\cite{chen2021evaluatinglargelanguagemodels}, and MBPP~\cite{mbpp2021} treat coding as a sequence transduction task, converting instructions directly into code without interactive execution. Recent efforts have expanded into interactive coding for Python, Bash, and other languages. Previous work~\cite{huang2022executionbasedevaluationdatascience, lai2022ds1000naturalreliablebenchmark} uses Python Jupyter Notebooks as an execution environment but faces challenges such as domain constraints, limited evaluation metrics, human-in-the-loop processes, or Python exclusivity. InterCode~\cite{intercode2023} provides a versatile framework supporting multiple languages and diverse settings with automatic execution-based evaluation. 

\textbf{Generation and Refinement:}
Recent studies in In-Context Learning~\cite{learningalgorithmincontextlearning2023, rethinkingroledemonstrationsmakes2022, explanationincontextlearningimplicit2022} enable models to quickly adapt to new context data at deployment time. Instead of relying on structured datasets, the context and queries are provided as sequences of text. The model uses this information to adjust its responses dynamically, allowing it to respond more accurately to future queries based on the immediate context, without needing traditional fine-tuning or parameter updates.
Recent studies in Chain-of-Thought (CoT) prompting~\cite{chainofthought2023, kojima2023largelanguagemodelszeroshot} enable models to perform multi-step reasoning using internal representations to answer questions in arithmetic, commonsense, and symbolic reasoning tasks. However, CoT reasoning is ungrounded in the external world, limiting its ability to update knowledge and causing fact hallucination and error propagation.
To address the limitations of CoT prompting, previous work has been done using ReAct framework and Plan-and-Solve prompting.
ReAct~\cite{react2023} prompts LLMs to generate reasoning traces and actions in an interleaved manner, enabling dynamic reasoning and plan adjustments (reason to act), while also interacting with external environments to refine reasoning (act to reason).
Plan-and-Solve~\cite{planandsolve2023} devises a plan to divide the entire task into smaller subtasks, and then carry out the subtasks according to the plan with detailed instructions mitigating calculation, missing step, and semantic misunderstanding errors. 


\textbf{Assessment and Evaluation:}
Recent work on code evaluation can be classified into four main approaches: (1) Match-based: Metrics like BLEU and CrystalBLEU~\cite{papineni2022bleu, eghbali2023crystalbleu} rely on n-gram matching to assess code similarity. (2) Embedding-based: Methods such as CodeBertScore~\cite{zhou2023codebertscore} measure similarity between generated and reference code by using token embeddings and contextual information. (3) Execution-based: These approaches evaluate code quality based on runtime correctness, using metrics like pass@$k$~\cite{kulal2019spoc, chen2021evaluatinglargelanguagemodels}.
(4) Prompt-based: Methods utilize LLMs for pairwise comparison (selecting the better of two codes), single answer grading (scoring a single code), and reference-guided grading (using a reference code if available)~\cite{zheng2023judging, liu2023geval, zhuo2024icescore}. CodeSift~\cite{codesift2024} uses a text-to-text approach, comparing the code’s textual representation with the task description to evaluate correctness.

==> CameraReady/LaTeX/tables/accuracy_userstudy.tex <==
% \begin{table*}[t]
% % \SetTblrInner{rowsep=0pt}
% \caption{Accuracy of code generation, assessment, and refinement based on User Study.}
% \label{tab:result}
% \begin{tblr}[]{
%     hline{1,2,Z} = {1pt},
%     hline{3,4} = {solid},
%     colspec={X[-1,c,m]X[-1,c,m]X[-1,c,m]X[-1,c,m]X[-1,c,m]X[-1,c,m]X[-1,c,m]},
%     rows={font=\footnotesize},
%     row{1} = {font=\footnotesize\bfseries},
%     % cell{2}{1}={r=2}{c},
% }

% Methods & 1st Pass Accuracy & Code Refinement & CodeSift Llama3\_70b HYBRID AND & CodeSift Llama3\_8b HYBRID AND & Improvement Llama3\_70b & Improvement Llama3\_8b \\ 
% strict  & 50/124            & 77/124          & 68/124                         & 76/124                        & 8 cases          & 13 cases         \\ 
% partial & 71/124            & 91/124          & 79/124                         & 83/124                        & 7 cases          & 12 cases         \\ 
% EA      & 29/124            & 45/124          & 55/124                         & 88/124                        & 4 cases          & 6 cases          \\ 
% \end{tblr}
% \end{table*}
